The exponentiated Hencky strain energy in modelling tire derived material for moderately large deformations

This work presents a hyper-viscoelastic model based on the Hencky-logarithmic strain tensor to model the response of a Tire Derived Material (TDM) undergoing moderately large deformations. TDM is a composite made by cold forging a mix of rubber fibers and grains, obtained by grinding scrap tires, and polyurethane binder. The mechanical properties are highly influenced by the presence of voids associated with the granular composition and low tensile strength due to the weak connection at the grain-matrix interface. For these reasons, TDM use is restricted to applications concerning a limited range of deformations. Experimental tests show that a central feature of the response is connected to highly nonlinear behavior of the material under volumetric deformation which conventional hyperelastic models fail in predicting. The strain energy function presented here is a variant of the exponentiated Hencky strain energy proposed by Neff et al., which for moderate strains is as good as the quadratic Hencky model and in the large strain region improves several important features from a mathematical point of view. The proposed form of the exponentiated Hencky energy possesses a set of parameters uniquely determined in the infinitesimal strain regime and an orthogonal set of parameters to determine the nonlinear response. The hyperelastic model is additionally incorporated in a finite deformation viscoelasticity framework that accounts for the two main dissipation mechanisms in TDMs, one at the microscale level and one at the macroscale level. The model is capable of predicting different deformation modes in a certain range of frequency and amplitude with a unique set of parameters with most of them having a clear physical meaning. Moreover, by comparing the predictions from the proposed constitutive model with experimental data we conclude that the new constitutive model gives accurate prediction.

==> table_figue_lists.tex <==
\section*{Table Captions}

Table 1: Tire Derived Material description.\\

Table 2: Initial guess for parameter identification procedure from tangents to the experimental data$^*$.\\

Table 3: Parameters - exponentiated-Hencky energy function.\\

\section*{Figure Captions}

Figure 1: Tire Derived Material. (a) TDM pad, (b) Close up view.\\

Figure 2: Comparison between shear stress corresponding to exponentiated Hencky energy $W_{\mathrm{eHm}}$, equation \eqref{taushear}, and experimental tests for different densities. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 3: Compression test procedure. First figure (a) shows strain history. Blue curve represent the true data. Red curve represents the assumed equilibrium response from the data. (a) Strain history, (b) TDM 500, (c) TDM 600, (d) TDM 800.  \\

Figure 4: Original image from the digital camera vs Image after processing for TDM 600. 0\%, 35\%, 70\%.\\

Figure 5: Non-linear Poisson's coefficient $\widehat{\nu}$ evaluated during compression tests.\\

Figure 6: Comparison between compression stress corresponding to modified exponentiated Hencky energy $W_{\mathrm{eHm}}$, equation \eqref{s} and \eqref{s2}, and experimental tests for different densities. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 7: Comparison between pseudo-volumetric response corresponding to equation \eqref{sigma} and experimental tests for different densities with $p \approx \sigma_{11}$. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 8: One dimensional rheological model for rate-dependent behavior of TDM.\\

Figure 9: Comparison between cyclic shear tests (markers) and the viscoelastic model based on the modified exponentiated Hencky energy $W^\mathrm{v}_{\mathrm{eHm}}$ (solid line), equation \eqref{functional}, for different frequencies at 100\% amplitude. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 10: Comparison between cyclic shear tests (markers) and the viscoelastic model based on the modified exponentiated Hencky energy $W^\mathrm{v}_{\mathrm{eHm}}$ (solid line), equation \eqref{functional}, for different amplitudes at 1 Hz. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 11: Comparison between cyclic compression tests (markers) and the viscoelastic model based on the modified exponentiated Hencky energy $W^\mathrm{v}_{\mathrm{eHm}}$ (solid line), equation \eqref{functional}, for different frequencies at 20\% amplitude. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 12: Comparison between cyclic compression tests (markers) and the viscoelastic model based on the modified exponentiated Hencky energy $W^\mathrm{v}_{\mathrm{eHm}}$ (solid line), equation \eqref{functional}, for different amplitudes at 1 Hz. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 13: Energy dissipation per hysteresis cycle in compression. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 14: Model parameter $\mu_A$ in the frequency and amplitude range. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 15: Model parameter $k_A$ in the frequency and amplitude range. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\

Figure 16: Model parameter $\mu_B$ in the frequency and amplitude range. (a) TDM 500, (b) TDM 600, (c) TDM 800.\\




